Paraphrasing in Affirmative Terms Improves Negation Understanding

Negation is a common linguistic phenomenon. Yet language models face challenges with negation in many natural language understanding tasks such as question answering and natural language inference. In this paper, we experiment with seamless strategies that incorporate affirmative interpretations (i.e., paraphrases without negation) to make models more robust against negation. Crucially, our affirmative interpretations are obtained automatically. We show improvements with CondaQA, a large corpus requiring reasoning with negation, and five natural language understanding tasks.

==> tables/affirmative_exampls.tex <==
\begin{tabularx}{l X X }
\toprule
Change Type & Negated sentence & Affirmative interpretation \\
\midrule
Adjective & The island became completely uninhabited by 1980 with the automation of the lighthouse. & The island became vacant by the 1980s because of the automation of the lighthouse. \\
\bottomrule
\end{tabularx}

==> tables/nluresults_old.tex <==
\small
\begin{tabular}{l c@{\hspace{.10in}} l r@{}l r@{}l r@{}l r@{}l r@{}l r@{}l r@{}l r@{}l r@{}l r@{}l}
	\toprule
	                                                                                                      & & & \multicolumn{4}{c}{\textbf{CmmnsnsQA}}                                                          & \multicolumn{4}{c}{\textbf{STS-B}}                                      & \multicolumn{4}{c}{\textbf{QNLI}}   & \multicolumn{4}{c}{\textbf{WiC}} & \multicolumn{4}{c}{\textbf{WSC}} \\
	\cmidrule(lr){4-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15} \cmidrule(lr){16-19} \cmidrule(lr){20-23} &  &  & Acc.                          &                           & F1                       &                         & Prsn                   &  & Sprmn &  & Acc. &  & F1   &  & Acc. &  & F1   &  & Acc. &  & F1   & \\
	\midrule w/out Affirmative Interpretations                                                            &  &  & 0.70                          &                           & 0.70                     &                         & 0.92                   &  & 0.92  &  & 0.93 &  & 0.93 &  & 0.71 &  & 0.71 &  & 0.69 &  & 0.69 & \\
	~~~~ w/o neg                                                                                          &  &  & 0.69                          &                           & 0.69                     &                         & 0.92                   &  & 0.92  &  & 0.93 &  & 0.93 &  & 0.72 &  & 0.71 &  & 0.67 &  & 0.67 & \\
	~~~~ w/ neg                                                                                           &  &  & 0.73                          &                           & 0.73                     &                         & 0.88                   &  & 0.88  &  & 0.92 &  & 0.92 &  & 0.67 &  & 0.66 &  & 0.71 &  & 0.71 & \\
	~~~~~~~~Important                                                                                     &  &  & 0.67                          &                           & 0.67                     &                         & 0.82                   &  & 0.85  &  & 0.85 &  & 0.78 &  & n/a   &  & n/a   &  & n/a   &  & n/a   & \\
	~~~~~~~~Unimportant                                                                                   &  &  & 0.80                          &                           & 0.80                     &                         & 0.88                   &  & 0.88  &  & 0.92 &  & 0.92 &  & 0.67 &  & 0.66 &  & 0.71 &  & 0.71 & \\
	\midrule \multicolumn{5}{l}{w/ Affirmative Interpretations}                                           &   \\
	~~obtained using T5-HB                                                                                &  &  & 0.72                          &                           & 0.72                     &                         & 0.92                   &  & 0.91  &  & 0.94 &  & 0.94 &  & 0.71 &  & 0.70 &  & 0.69 &  & 0.68 & \\
	~~~~ w/o neg                                                                                          &  &  & 0.72                          &                           & 0.72                     &                         & 0.92                   &  & 0.92  &  & 0.94 &  & 0.94 &  & 0.71 &  & 0.71 &  & 0.63 &  & 0.62 & \\
	~~~~ w/ neg                                                                                           &  &  & 0.74                          &                           & 0.74                     &                         & 0.88                   &  & 0.88  &  & 0.93 &  & 0.92 &  & 0.70 &  & 0.70 &  & 0.75 &  & 0.74 & \\
	~~~~~~~~Important                                                                                     &  &  & 0.70                          &                           & 0.70                     &                         & 0.83                   &  & 0.84  &  & 0.95 &  & 0.89 &  & n/a   &  & n/a   &  & n/a   &  & n/a   & \\
	~~~~~~~~Unimportant                                                                                   &  &  & 0.79                          &                           & 0.80                     &                         & 0.87                   &  & 0.88  &  & 0.93 &  & 0.92 &  & 0.70 &  & 0.70 &  & 0.75 &  & 0.74 & \\
	~~obtained using T5-CG                                                                               &  &  & 0.71                          &                           & 0.71                     &                         & 0.92                   &  & 0.92  &  & 0.94 &  & 0.94 &  & 0.73 &  & 0.73 &  & 0.72 &  & 0.71 & \\
	~~~~ w/o neg                                                                                          &  &  & 0.71                          &                           & 0.71                     &                         & 0.93                   &  & 0.92  &  & 0.94 &  & 0.94 &  & 0.74 &  & 0.73 &  & 0.69 &  & 0.68 & \\
	~~~~ w/ neg                                                                                           &  &  & 0.74                          &                           & 0.74                     &                         & 0.88                   &  & 0.88  &  & 0.93 &  & 0.92 &  & 0.70 &  & 0.70 &  & 0.75 &  & 0.75 & \\
	~~~~~~~~Important                                                                                     &  &  & 0.69                          &                           & 0.69                     &                         & 0.82                   &  & 0.87  &  & 0.95 &  & 0.89 &  & n/a   &  & n/a   &  & n/a   &  & n/a   & \\
	~~~~~~~~Unimportant                                                                                   &  &  & 0.80                          &                           & 0.80                     &                         & 0.88                   &  & 0.88  &  & 0.93 &  & 0.92 &  & 0.70 &  & 0.70 &  & 0.75 &  & 0.75 & \\
	\bottomrule
\end{tabular}
